Unleashing OpenTitan's Potential: a Silicon-Ready Embedded Secure Element for Root of Trust and Cryptographic Offloading

The rapid advancement and exploration of open-hardware RISC-V platforms are driving significant changes in sectors like autonomous vehicles, smart-city infrastructure, and medical devices. OpenTitan stands out as a groundbreaking open-source RISC-V design with a comprehensive security toolkit as a standalone system-on-chip (SoC). OpenTitan includes Earl Grey, a fully implemented and silicon-proven SoC, and Darjeeling, announced but not yet fully implemented. Earl Grey targets standalone SoC implementations, while Darjeeling is for integrable implementations. The literature lacks a silicon-ready embedded implementation of an open-source Root of Trust, despite lowRISC's efforts on Darjeeling. We address the limitations of existing implementations by optimizing data transfer latency between memory and cryptographic accelerators to prevent under-utilization and ensure efficient task acceleration. Our contributions include a comprehensive methodology for integrating custom extensions and IPs into the Earl Grey architecture, architectural enhancements for system-level integration, support for varied boot modes, and improved data movement across the platform. These advancements facilitate deploying OpenTitan in broader SoCs, even without specific technology-dependent IPs, providing a deployment-ready research vehicle for the community. We integrated the extended Earl Grey architecture into a reference architecture in a 22nm FDX technology node, benchmarking the enhanced architecture's performance. The results show significant improvements in cryptographic processing speed, achieving up to 2.7x speedup for SHA-256/HMAC and 1.6x for AES accelerators compared to the baseline Earl Grey architecture.

==> sections/tables/area-occupation.tex <==
\begin{table}[t]
    \centering
    \caption{Power consumption and Area occupation}
    % \begin{tabular}{|c|c|c|c|c|c|} 
    \begin{tabular}{lrr} 
        \toprule
        \multirow{2}{*}{Component} & \multicolumn{1}{c}{Area} & \multicolumn{1}{c}{Max Freq}  \\ 
                          & \multicolumn{1}{c}{[$mm^2$]}   & \multicolumn{1}{c}{[$MHz$]}  \\ 
        \midrule
        Top Module       & 7.28       & 450 \\ %\hline
        Dual-core CVA6   & 0.98       & 900 \\ %\hline
        PMCA             & 1.56       & 400 \\ %\hline
        HyperRam Ctrl    & 0.32       & 450 \\ %\hline
        Opentitan        & 1.70       & 500 \\ %\hline
        Total            & 7.28       & -   \\ %\hline
        \bottomrule
    \end{tabular}
    \label{tab:area_freq}
\end{table}


==> sections/tables/mbox_mmap.tex <==
\begin{table}[t]
    \centering
    \caption{This table shows the SCMI-compliant mailbox register file's memory map}
    % \begin{tabular}{|c|c|c|c|c|c|} 
    \begin{tabular}{lll} 
        \toprule
        \multirow{1}{*}{Register} & \multicolumn{1}{c}{Offset}  & \multicolumn{1}{c}{Size}  \\ 
        \midrule
        Reserved         & 0x0    & 0x4   \\ %\hline
        Channel status   & 0x4    & 0x4   \\ %\hline
        Reserved         & 0x8    & 0x8   \\ %\hline
        Channel flags    & 0x10   & 0x4   \\ %\hline
        Length           & 0x14   & 0x4   \\ %\hline
        Message header   & 0x18   & 0x4   \\ %\hline
        Message Payload  & 0x1C   & N     \\ %\hline
        \bottomrule
    \end{tabular}
    \label{tab:mbox_mmap}
\end{table}


==> sections/tables/results.tex <==
\begin{table}
    \centering
    \caption{To Do}
    \label{table:results}
    \begin{tabular}{cr*{9}{>{\raggedleft\let\newline\\\arraybackslash}p{.35in}}}

        \toprule

        \multicolumn{2}{c}{\multirow{2}{*}{Payload}} & \multicolumn{3}{c}{SHA-256} & \multicolumn{3}{c}{HMAC} & \multicolumn{3}{c}{AES-256-CBC} \\
        \cmidrule(lr{0.5em}){3-5}
        \cmidrule(lr{0.5em}){6-8}
        \cmidrule(lr{0.5em}){9-11}
                               &                     & Base & Xbar & DMA           & Base & Xbar & DMA        & Base & Xbar & DMA               \\

        \midrule

        \multirow{6}{*}{\rotatebox[origin=c]{90}{System RAM}}
        &    64 B & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   256 B & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   1 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   4 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &  16 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &  64 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

        \midrule

        \multirow{4}{*}{\rotatebox[origin=c]{90}{OpenTitan}}
        &    64 B & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   256 B & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   1 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        &   4 kiB & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
     
        \bottomrule

    \end{tabular}
\end{table}
